Rosko: Row Skipping Outer Products for Sparse Matrix Multiplication Kernels

We propose Rosko -- row skipping outer products -- for deriving sparse matrix multiplication (SpMM) kernels in reducing computation and memory access requirements of deep neural networks (DNNs). Rosko allows skipping of entire row computations during program execution with low sparsity-management overheads. We analytically derive sparse CPU kernels that adapt to given hardware characteristics to effectively utilize processor cores and minimize data movement without the need for auto-tuning or search space exploration. Rosko can be integrated with other outer product scheduling methods, allowing them to leverage row skipping by using Rosko's packing format to skip unnecessary computation. Rosko kernels outperform existing auto-tuning and search-based solutions as well as state-of-the-art vendor-optimized libraries on real hardware across a variety of neural network workloads. For matrices with sparsities ranging from 65% to 99.8% typically found in machine learning, Rosko kernels achieve up to a 6.5x runtime reduction on Intel and ARM CPUs.

==> old/abstract.tex <==


% Matrix multiplication is a key computation in deep neural networks (DNNs).
% Leveraging sparsity is a common way to reduce computation and memory requirements for DNNs.
% However, as sparsity increases, there is a tradeoff between enabling efficient hardware support and maintaining high inference accuracy.
% By mapping DNN computations to outer product matrix multiplications, we can exploit sparsity across filters within neural network layers.
% We present Rosko, a scheme that uses row-skipping outer products in performing efficient sparse-dense matrix multiplication.
% Rosko takes advantage of a novel sparsity pattern which, when applied to DNN weights, can achieve high sparsity while maintaining high inference accuracy.

% Rosko kernels outperform competing libraries, including Intel oneMKL and ARM Compute Library, for matrices with sparsities ranging from 75.9% and 99.8%.
% At 95% sparsity, Rosko kernels achieve up to a 6.5x reduction in runtime on an Intel CPU and 4.7x reduction in runtime on an ARM CPU.

\begin{comment}
Matrix multiplication is a key computation in deep neural networks (DNNs).
Leveraging sparsity is a common way to reduce computation and memory requirements for DNNs.
However, as sparsity increases, there is a tradeoff between enabling efficient hardware support and maintaining high inference accuracy.
By mapping DNN computations to outer product matrix multiplications, we can exploit sparsity across filters within neural network layers.
We present Rosko, a scheme that uses \textit{row-skipping outer products} in performing efficient sparse-dense matrix multiplication.
Rosko takes advantage of a novel sparsity pattern which, when applied to DNN weights, can achieve high sparsity while maintaining high inference accuracy.

Rosko kernels outperform competing libraries, including Intel oneMKL and ARM Compute Library, for matrices with sparsities ranging from 75.9\% and 99.8\%.
At 95\% sparsity, Rosko kernels achieve up to a 6.5x reduction in runtime on an Intel CPU and 4.7x reduction in runtime on an ARM CPU.
% for dense and sparse matrix multiplication perform poorly for
%up to a 3x reduction in runtime for 95\% sparsity and 4.7x for 99\% sparsity.
%is a balanced approach that enables high accuracy and sparsity while still allowing for efficient hardware
% However, unstructured pruning is difficult to leverage and structured pruning will result in degraded accuracy.
% Balanced sparsity, induces unstructured sparsity within structured groups of elements, supporting simpler hardware acceleration from structured sparsity while maintaining a similar accuracy to unstructured sparsity.support.
\end{comment}

\begin{comment}

%$N$:$M$ sparsity, has unstructured sparsity within each group of $M$ elements, creating a hybrid between structured and unstructured.
%Hard to achieve good balance. Our paper has a solution based on outer products
% Sparsity can be induced in the weight matrices of neural networks during training via structured or unstructured pruning.% techniques.
% While structured pruning is straightforward to accelerate, with minimal overhead, it may result in degraded DNN inference accuracy.
% On the other hand, unstructured pruning is able to achieve good inference accuracy and high levels of weight sparsity, but this sparsity is difficult to leverage on modern CPU hardware.
% Balanced sparsity, also known as $N$:$M$ sparsity, has unstructured sparsity within each group of $M$ elements, creating a hybrid between structured and unstructured.
However, there is a tradeoff between achieving efficient hardware support and high accuracy when deciding how fine-grained structured pruning should be.
[N:M sparsity] is a balanced approach that enables high accuracy and sparsity while still allowing for efficient hardware support.

%outer product novelty. Give numbers
Existing CPU libraries for dense and sparse matrix multiplication perform poorly for sparsity levels commonly found in deep learning.
% Zero-skipping is a common technique for increasing computation throughput of matrix multiplication.
% Keeping track of skipped computation introduces complicated indexing which impacts performance for matrices that are less sparse.
% Unstructured pruning is able to achieve high levels of sparsity, but this sparsity is difficult to leverage.
% Structured pruning requires minimal overhead and is straightforward to accelerate, [but results in degraded performance].
We present Rosko, a scheme that incorporates a unique form of [outer product $N$:$M$ sparsity] as well as row-skipping outer product kernels that can leverage that sparsity.
% Rosko addresses the zero-skipping problem with outer product sparsity by skipping rows of computation when there is a a zero.
We demonstrate high sparsity is achievable with minimal accuracy loss using Rosko pruning.
Using multiple DNN benchmarks, we evaluate Rosko kernels on a desktop and embedded CPU.
\end{comment}

==> old/background.tex <==
%Several libraries for SpMM exist on different architectures. 
% In this paper, we focus specifically on inference, where weight sparsity is known ahead of time.
% Prior to inference we have to introduce some amount of sparsity.
% Sparsity can be introduced during training or as a step after training is complete.
% In this paper we introduce sparsity during training by pruning, setting values to zero.

% \subsection{DNN Weight Pruning}
% Increasing the number of zeros, or sparsity, in a DNN can reduce the amount of computation needed when multiplication with zero operands may be skipped.
% Weight pruning is commonly used for increasing sparsity in a DNN by setting weight values to zero.
% Pruning can be applied at the level of individual weight elements (unstructured) or to groups of elements (structured) at varying granularities \cite{anwar2017structured}.
% These groups can be filters, channels, or entire layers of a network.
% Approaches to structured pruning include using LASSO or $\ell_1$ channel selection \cite{he2015deep, liu2017learning} to determine pruning targets.

%We motivate the use of outer products in Rosko by analyzing the arithmetic intensity (AI) attainable with outer product MM versus inner product MM. AI for a given operation is defined as the ratio of computation throughput to external memory bandwidth. By increasing AI, one can utilize additional processing cores to increase throughput without requiring a proportional increase in memory bandwidth.

% By increasing this ratio, or arithmetic intensity (AI), one can utilize additional processing cores to increase throughput without requiring a proportional increase in memory bandwidth.

%$C$ IO is more than $A$ and $B$, so we allocate more memory to $C$.
%In general, the fewer tiles 

% This IO can vary with computation schedule such as inner vs. outer product schedules.
%, as we will demonstrate in \Cref{sec:outer_io} and \Cref{sec:inner_io}.

%may be skipped without checking for individual values.
% In this paper we show how unstructured pruning within a group of values can result in a hardware friendly sparsity distribution with similar impact on accuracy to unstructured pruning.

==> old/intro.tex <==
\begin{comment}
Paper outline: \\
- Machine learning and matrix multiplication
- Sparsity within the models implies sparse matrix multiplications
- There are many methods for inducing sparsity. Give a brief intro to unstructured and structured methods
- Unstructured pruning came first due to its simplicity. However it is hard to leverage because zeros are distributed randomly. 
- To address this people came up with structured pruning which directly created smaller networks
- However, [it is difficult to retain accuracy with structured pruning at the same level of sparsity as unstructured pruning] % structured pruning may create a smaller dense problem
- To address this gap people have introduced approaches such as balanced sparsity with the flexibility of unstructured sparsity within each group while maintaining predictable structure and distribution of non-zero elements across groups to reduce indexing overhead.

- Existing sparse kernels, which are often used in scientific applications, are tuned for extremely sparse matrices [cite]. In machine learning we often see less sparse matrices, for example in the range of 50-99\%.
% - To maximize performance for extremely sparse matrices one must use specific structures to keep track of the very few non-zero elements
- For the [ML sparsity] matrices the overhead becomes significant (Vikas runtime analysis)
- Dense libraries do not benefit from increased sparsity
- To address this gap

\end{comment}
% The Rosko scheme takes a similar approach to N:M sparsity but groups elements based on outer product formulations instead of inner products.

% Approach: section on outer product takes advantage of sparsity
% mention cake scheduling

% Rosko consists of several components: Rosko kernels which take advantage of a novel computation structured sparsity that is obtained via the Rosko scheme.
% The Rosko scheme is a pruning method for creating DNNs with high accuracy and a structure that can be leveraged by Rosko kernels.
% DNN matrices often do not fit into memory, requiring redundant memory accesses.
% Maximizing computation throughput for SpMM requires two complimentary approaches: reducing memory accesses through scheduling and leveraging sparsity by zero skipping.
% However, alone Rosko kernels don't compute an entire MM, instead they need to be implemented with a schedule such as CAKE or Goto's algorithm. 

%Rosko kernels are performed from a higher level of memory which often results in matrices that must be partitioned into smaller computations.
% A DNN trained using the Rosko scheme will be load balanced because every outer product group will have the same amount of sparsity. % when groups are distributed between parallel Rosko kernels:

%In machine learning, matrices are often between 50\% and 99\% sparsity.

% As mentioned by \cite{} dense MM kernels are used. there is a lack of good sparse kernels for sparsities below 99.9\%, 

%by presenting an approach that leverages outer product formulations of matrix multiplication to facilitate the skipping of zero computations.
 % range of sparsity for intel and arm

==> old/motivation.tex <==
\begin{comment}
In an outer product between a column vector and row vector, the results of each row of computation depends on only one element from the column vector.
Thus, we can determine whether to skip a whole row of computation simply by checking if an element is zero, as shown in \Cref{fig:rosko_scheme}.
Rows that are not skipped can be computed without additional checks.
Thus, outer products are suitable for leveraging input column sparsity.

We use this property to improve outer product based matrix multiplication with sparse column vectors inputs.
For a tile MM using outer products, once an element has been skipped, we can ensure it will no longer be needed for any remaining tile computations (i.e., other outer products).
In contrast, when using inner products, we would need to repeatedly check individual elements to determine which operations to skip. 
% Atomicity of vector operations means you are applying the same operation to many elements in parallel. Inner product can't leverage this. If you try to leverage based on individual elements you can't skip
% An outer product can be computed as a set of vector register operations. 
% It is easy to skip an entire vector operation rather than an individual element operation. Because of that we can take advantage of vector hardware more easily.

For any general purpose SIMD architectures, row-skipping outer products are a simple scheme to implement and do not require hardware modifications.
Inputs to row-skipping outer products need only a simple indexing scheme (described in \Cref{sec:rosko_scheme}), so there is minimal unpacking and indexing overhead.
% For example, the Nvidia A100 has specialized hardware to perform sparse inner products.
% when one of the operands to an inner product is sparse it is not possible to perform a single instruction which skips zeros.
% Also there would be no speedup.
% requires multiple checks within a single vector instruction.
% do re
% [something] allows us to compute rows using vector registers.
% Additionally, Rosko does not require remapping indices beyond the inner kernels and therefore has low packing overhead.
%as is demonstrated by our implementation on multiple CPU architectures.
% Other approaches such as [dual side tensor] require dedicated hardware.


%- Lightweight

%- Flexible
\end{comment}

==> old/related_work.tex <==
\section{Related Works}
\label{sec:related_works}

In this section, we compare Rosko to prior pruning approaches for achieving fine-grained structured sparsity amenable to hardware acceleration, 

\begin{comment}
\subsection{Achieving Fine-grained Structured Sparsity}
\label{sec:nm_sparsity}
As sparsity increases, there is a tradeoff between enabling granular sparsity and maintaining efficient hardware support.
Prior works such as \cite{yu2017scalpel} employ pruning techniques that ensure dense, contiguous groups of non-zero weights, sized to and aligned to the width of SIMD hardware (e.g., vector registers).
While such pruning enables efficient use of SIMD hardware, it limits how granular sparsity can be while maintaining high model accuracy.

% [Standard approaches to parallelizing matrix multiplication, such as tiling, will not ensure equally distributed workloads for each processor.]
% Fine-grained structured pruning leverages aspects of both unstructured and structured pruning
Balanced sparsity \cite{yao2019balanced}, also known as $N$:$M$ sparsity, aligns weights to groups of size $M$.
There are $N$ non-zero weights for each continuous group of $M$ weights,  with $N < M$.
Approaches such as \cite{mishra2021accelerating} specifically target 2:4 sparsity ($N=2, M=4$) to allow specialized hardware support (e.g., Nvidia A100's Sparse Tensor Cores \cite{tensor}).

With Rosko, we obtain a matrix with a target sparsity (e.g., 90\%) and sparse columns through iterative pruning during training.
%to obtain a matrix $A$ with sparse columns satisfying a certain sparsity objective.
Since the pruned elements are from column input vectors, we may vary the size of the columns without restricting our pruning granularity to hardware SIMD lengths (\Cref{sec:training_for_scs}) {or specific sparsities (e.g., 50\% in 2:4 sparsity).}
% $N$:$M$ sparsity enables the flexibility of unstructured sparsity within each group while restricting the distribution of non-zero elements across groups to reduce indexing overhead.
% In contrast, our pruning scheme results in \textit{balanced outer product sparsity}, a form of $N$:$M$ sparsity with \textit{column groups} to facilitate row skipping outer product computations, as described in \Cref{sec:training_for_scs}.





Under the above approaches, nonzeros of sparse inputs may not be evenly distributed, causing workload imbalances when using multiple processing elements in parallel.
Hardware such as \cite{2020nvidia} {avoid imbalances by using input formats} with a specific sparsity type (e.g., 2:4 sparsity). %for performing sparse dot products on sparse tensor cores.
Most recently, approaches such as \cite{qin2020sigma} introduce additional routing logic to address dynamic workload balancing { support for sparse input formats}.

Outer product column sparsity of this paper enables efficient zero-skipping.
When a column input vector is sparse but not completely empty, Rosko skips computations for the rows in outer product corresponding to the zero elements in the column input.
Moreover, for outer products with a completely empty input column, Rosko kernels can avoid loading the dense input row vector.
\end{comment}


==> old/rop_pruing.tex <==
\section{Pruning for ROP Sparsity}
\label{sec:training}
Targeting a specific $N$:$M$ sparsity helps load balancing for ROP kernels across multiple processing cores in parallel.

During training, we iteratively prune to several specified sparsity levels and evaluate accuracy performance, as shown in \Cref{fig:training}.

% We implement a version of balanced sparsity that groups elements into groups and prunes within the group.
%By pruning within a group we are able to have an exact distribution of sparsity for each inner kernel.
% By selecting the group size, we are able to control the distribution of sparsity of the MM such that we can load balance between inner kernels.
% ROP training yields an exact amount of sparsity for each inner kernel.

Every 10 epochs, weights are pruned to increase sparsity.
Weights with the smallest magnitude are pruned until the desired sparsity is met.
We prune according to $N$:$M$ sparsity if there are $M$ elements in a group, the $N$ weights with the lowest magnitude are set to 0.
After the desired sparsity is reached the network is trained until a total of 200 epochs has passed (including when pruning was occurring).

\subsection{Comparison with Structured and Unstructured Pruning}
The ROP training approach allows us to leverage sparsity without a significant loss in test accuracy compared to unstructured pruning.
The accuracy remains similar to unstructured pruning because we the sparsity is unstructured within a group.
Group sizes are large enough that accuracy doesn't decrease like structured sparsity.
% Say something out how we have the benefit of strucuted sparsity without the acc penalty
Compared to structured sparsity induced by iterative magnitude pruning during training. 

\Cref{fig:training} shows that the desired ROP sparsity pattern IS achieved without sacrificing accuracy.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/training.png}
    \caption{CIFAR-10 and CIFAR-100 Test Accuracy for Resnet-18 and Resnet-50 with ROP pruning has little to no loss in model accuracy compared to unstructured pruning for sparsity levels ranging from 44\%-88\%. ROP pruning does not have the same accuracy drop as the more restrictive structured pruning of 3x3 blocks for sparsities greater than 50\%.}
    \label{fig:training}
\end{figure}

==> reorder.tex <==
\begin{figure}[h]
    \centering
    \subfloat{\label{fig:reorder_a}{\includegraphics[scale=0.38]{figures/figa.pdf}}}
    \subfloat{\label{fig:reorder_b}{\includegraphics[scale=0.38]{figures/figb.pdf}}}
    \subfloat{\label{fig:reorder_c}{\includegraphics[scale=0.38]{figures/figc.pdf}}}
\caption{
    {
	Reordering outer product columns by density to reduce the performance impact of CPU speculation.
	(a) A $6\times16$ outer product tile with random sparsity. Colored squares depict nonzero values, and all nonzero values in the same row have the same color.
	(b) We pack non-zeros in each column into contiguous segments. We use an indexing array containing the $m$ dimension index of each nonzero value in the weight tile to write the result row to the correct row of the result matrix. Since the number of nonzero elements in each column vector is unknown at compile time, the CPU cannot predict the bound of the $m$ dimension loop of each outer product. When we reorder columns according to their density in (c), the CPU can more easily predict the loop bound for each outer-product, reducing speculation penalty.
    }
} \label{fig:reorder}
\end{figure}



==> training.tex <==
\begin{figure*}[ht]
    \centering
    \subfloat{\label{fig:vgg}{\includegraphics[height=0.18\textheight]{figures/training_vgg.pdf}}}
    \subfloat{\label{fig:mobilenet}{\includegraphics[height=0.18\textheight]{figures/training_mobilenet.pdf}}}
    \subfloat{\label{fig:resnet}{\includegraphics[height=0.18\textheight]{figures/training_resnet.pdf}}}
\caption{
    Rosko pruning shows little to no loss in model accuracy compared to unstructured pruning after 200 epochs. % for sparsity levels ranging from 40\%-95\%
    For sparsities greater than 50\%, Rosko pruning maintains higher accuracy compared to structured pruning using 3x3 blocks. 
    (a) Rosko pruning for VGG-19,
    (b) Rosko Pruning for MobileNetV2, and
    (c) Rosko pruning for ResNet-18 and ResNet-50.
} \label{fig:training}
\end{figure*}

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/training_resnet.pdf}
    \caption{CIFAR-10 and CIFAR-100 Test Accuracy for ResNet-18 and ResNet-50.
    Rosko pruning shows little to no loss in model accuracy compared to unstructured pruning for sparsity levels ranging from 40\%-95\%.
    For sparsities greater than 50\%, Rosko pruning maintains higher accuracy compared to structured pruning using 3x3 blocks.}
    \label{fig:training}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/training_mobilenet.pdf}
    \caption{CIFAR-10 and CIFAR-100 Test Accuracy for MobileNetV2}
    \label{fig:training_mobilenet}
\end{figure}
\end{comment}
